MetaComp: Learning to Adapt for Online Depth Completion

Relying on deep supervised or self-supervised learning, previous methods for depth completion from paired single image and sparse depth data have achieved impressive performance in recent years. However, facing a new environment where the test data occurs online and differs from the training data in the RGB image content and depth sparsity, the trained model might suffer severe performance drop. To encourage the trained model to work well in such conditions, we expect it to be capable of adapting to the new environment continuously and effectively. To achieve this, we propose MetaComp. It utilizes the meta-learning technique to simulate adaptation policies during the training phase, and then adapts the model to new environments in a self-supervised manner in testing. Considering that the input is multi-modal data, it would be challenging to adapt a model to variations in two modalities simultaneously, due to significant differences in structure and form of the two modal data. Therefore, we further propose to disentangle the adaptation procedure in the basic meta-learning training into two steps, the first one focusing on the depth sparsity while the second attending to the image content. During testing, we take the same strategy to adapt the model online to new multi-modal data. Experimental results and comprehensive ablations show that our MetaComp is capable of adapting to the depth completion in a new environment effectively and robust to changes in different modalities.

==> outline/others.tex <==
Currently, Depth completion has been considered as a two stage task in many researches \cite{}.
A coarse dense depth is firstly produced from the sparse input and then is taken as input with the image to predict the final dense depth.
The sparse-to-coarse operation makes the core network not need to directly adapt to sparse points and enhances the robustness of the whole model to sparse inputs to to a certain extent.
Similarly, We regard the depth completion as a two stage task and adopt Unguided Normalized CNNs \cite{ncnn} as our sparse-to-coarse module.
To increase the the robustness of the model to sparse inputs, we propose a novel meta-learning algorithm to learn to adapt to sparse points(LAS).
LAS has two steps: 1) Adapt the sparse-to-model module to sparse inputs. 
This step is aimed to improve the adaptability of the model to sparse inputs with different patterns.
2) Adapt the core network to different image input.
The purpose of the step is to enhance the model generalization to 
Several researches \cite{sfm, dig, ss2d} project the image of near frame to the current frame through relative pose and take the error between the original image and projected image as supervision.
Inspired by \cite{sfm, dig, ss2d}, we project the sparse map of the previous frame to the next frame that increases the density of the sparse map of the next frame to obtain a stronger prior for better online adaptation.
However, a depth completion model is sensitive to the changes of sparse inputs, and sparse projecting changes the pattern of sparse inputs and introduces noise points which results in a perturbation to the model.
Therefore, how to balance the prior and perturbation brought by projected sparse points is the core issue to our work.

\IncMargin{1em}
\begin{algorithm}
 
    \SetAlgoNoLine 
    \SetKwInOut{Input}{\textbf{Require}}
 
\Input{\\
        Training video sequence: $D_v=\{i_1,i_2,...,i_N\}$;\\
        Hyper-parameters: $\alpha, \beta, n$\\
        Model parameters to be trained: $\theta$
        }
    \BlankLine
 
    initialize $\theta$\\
    $s \leftarrow 0$\\
    \While{$s\leq N-n$}{
        ${\theta}_s \leftarrow \theta $\\
        $L_s \leftarrow 0$\\
        \For {$t \leftarrow s,...,s+n-1$}{
            ${\theta}_{t+1} \leftarrow {\theta}_t -\bigtriangledown_{{\theta}_t}L_u(\theta_t, i_t)$\\
            $L_s \leftarrow L_s+L_u(\theta_{t+1}, i_{t+1})$ 
        }
        $\theta \leftarrow \theta - \beta\bigtriangledown_\theta L_s$\\
        $s \leftarrow s+n$
    }
    \caption{Basic meta-learning for depth completion}
\end{algorithm}
\DecMargin{1em}
